Surgery obstructions and Heegaard Floer homology

Using Taubes' periodic ends theorem, Auckly gave examples of toroidal and hyperbolic irreducible integer homology spheres which are not surgery on a knot in the three-sphere. We give an obstruction to a homology sphere being surgery on a knot coming from Heegaard Floer homology. This is used to construct infinitely many small Seifert fibered examples.

==> proof.tex <==
\section{Proof of Theorem~\ref{thm:main}}
Irreducibility of $Y_p$ is clear since all Seifert homology spheres are irreducible REFERENCE.  \\
Surgery on a two-component link (Hoffman-Walsh) and give the picture (but no proof). \\
For the proof of weight one, see.  \\
$d(Y_p) = -p$ is computed in PLUMBING.  Reference Ozsv\'ath-Szab\'o for rational homology cobordance.  (Auckley's examples have $d = 0$ since they are homology cobordant to $S^3$) \\
In Proposition ? we prove that $\rank (\ker U)_0 + 1 = \rank HF^+_0(Y)$.  Now, we prove that that implies $U \cdot (\HFred)_0 = 0$.  This follows from structure of Heegaard Floer homology for rational homology spheres.  \\
The result now follows by applying Theorem~\ref{thm:?}.  \qedhere

